Embracing Imperfect Datasets: A Review of Deep Learning Solutions for Medical Image Segmentation

The medical imaging literature has witnessed remarkable progress in high-performing segmentation models based on convolutional neural networks. Despite the new performance highs, the recent advanced segmentation models still require large, representative, and high quality annotated datasets. However, rarely do we have a perfect training dataset, particularly in the field of medical imaging, where data and annotations are both expensive to acquire. Recently, a large body of research has studied the problem of medical image segmentation with imperfect datasets, tackling two major dataset limitations: scarce annotations where only limited annotated data is available for training, and weak annotations where the training data has only sparse annotations, noisy annotations, or image-level annotations. In this article, we provide a detailed review of the solutions above, summarizing both the technical novelties and empirical results. We further compare the benefits and requirements of the surveyed methodologies and provide our recommended solutions. We hope this survey article increases the community awareness of the techniques that are available to handle imperfect medical image segmentation datasets.

==> chapters/unsupervised.tex <==
When faced the a complete absence of any annotations, unsupervised approaches have been used to perform medical image segmentation as in the case of \cite{zhang2018self} that learns to segment lymphangioleiomyomatosis (LAM) cysts from chest CT scans in an unsupervised fashion. They generate the initial ground truth using K-means clustering followed by graph cuts refinement. The model first learns to segment the cysts using this ground truth and is then kept frozen to produce new ground truth masks which will will be used to train the second stage. The model is repeatedly trained self-learn and incrementally improve the segmentation results.
